The Local Learning Coefficient: A Singularity-Aware Complexity Measure

The Local Learning Coefficient (LLC) is introduced as a novel complexity measure for deep neural networks (DNNs). Recognizing the limitations of traditional complexity measures, the LLC leverages Singular Learning Theory (SLT), which has long recognized the significance of singularities in the loss landscape geometry. This paper provides an extensive exploration of the LLC's theoretical underpinnings, offering both a clear definition and intuitive insights into its application. Moreover, we propose a new scalable estimator for the LLC, which is then effectively applied across diverse architectures including deep linear networks up to 100M parameters, ResNet image models, and transformer language models. Empirical evidence suggests that the LLC provides valuable insights into how training heuristics might influence the effective complexity of DNNs. Ultimately, the LLC emerges as a crucial tool for reconciling the apparent contradiction between deep learning's complexity and the principle of parsimony.

==> images/mnist_expt_description_points.tex <==

Experiment Details:
------------------
- Dataset: MNIST
  - Training samples: 60000
  - Testing samples: 10000

- Network: Multi-layer Perceptron (MLP)
  - Number of parameters: 1863690
  - Hidden layer sizes: 1024, 1024

- Training:
  - Optimizer: SGD and Entropy-SGD
  - Learning rate: 0.01
  - Number of epochs: 200
  - Batch size: 512

- Stochastic Gradient Langevin Dynamics (SGLD) Parameters:
  - Gamma: 100.0
  - Number of iterations: 400
  - Number of chains: 4
  - Noise standard deviation: 1e-05

Num experiment repeats: 80


==> images/mnist_expt_description_prose.tex <==

In this experiment, we trained a feedforward ReLU on the MNIST dataset. The dataset consists of 60000 training samples and 10000 testing samples. The network is designed with 2 hidden layers having sizes [1024, 1024], and it contains a total of 1863690 parameters. 

For training, we employed two different optimizers, SGD and EntropySGD, with learning rate of 0.01 and batch size of 512. The network is trained for 200 epochs. The number of epoch is chosen so that the classification error rate on the training set for both optimizers falls to zero. 

The localizing prior scale parameter $\gamma$ is set to 100.0
The hyperparameters used for SGLD approximate posterior sampling are as follow: $\epsilon$ is set to 1e-05 and each of four independent SGLD chains is run for 400 iterations.

The experiments are repeated for 80 RNG seeds. 


==> images/table_lambdahat_small.tex <==
\begin{tabular}{llll}
\toprule
monomial & $\lambda(\wstar)$ & MCMC $\hatlambdawstar$ & SGLD $\hatlambdawstar$\\
\midrule
$w_1^1w_2^3$ & 0.17 &  0.12 ( 0.04) &  0.11 ( 0.07) \\
$w_1^1w_2^2$ & 0.25 &  0.19 ( 0.11) &  0.14 ( 0.12) \\
$w_1^0w_2^1$ & 0.50 &  0.41 ( 0.12) &  0.45 ( 0.11) \\
$w_1^1w_2^0$ & 0.50 &  0.43 ( 0.12) &  0.47 ( 0.13) \\
\bottomrule
\end{tabular}


==> images/table_nu_small.tex <==
\begin{tabular}{lll}
\toprule
monomial & MCMC & SGLD\\
\midrule
$w_1^1w_2^3$ &  0.17 ( 0.03) &  0.14 ( 0.05) \\
$w_1^1w_2^2$ &  0.32 ( 0.16) &  0.23 ( 0.09) \\
$w_1^0w_2^1$ &  0.50 ( 0.04) &  0.54 ( 0.04) \\
$w_1^1w_2^0$ &  0.49 ( 0.03) &  0.53 ( 0.05) \\
\bottomrule
\end{tabular}


==> images/toypotential_table_of_results.tex <==
\begin{tabular}{lllrrrrrrrrrrrr}
\toprule
monomial & prior & $\lambda$ & \multicolumn{4}{r}{MCMC} & \multicolumn{4}{r}{SGLD ($\epsilon=0.0001$)} & \multicolumn{4}{r}{SGLD ($\epsilon=0.0005$)} \\
 &  &  & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$V_n^{\beta^*}/2$} & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$V_n^{\beta^*}/2$} & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$V_n^{\beta^*}/2$} \\
 &  &  & mean & std & mean & std & mean & std & mean & std & mean & std & mean & std \\
\midrule
$w_1^1w_2^3$ & $w_1^1w_2^0$ & 0.17 & 0.17 & 0.01 & 8.03 & 0.36 & 0.14 & 0.10 & 6.55 & 3.49 & 0.16 & 0.05 & 8.51 & 2.09 \\
$w_1^1w_2^3$ & uniform & 0.17 & 0.12 & 0.04 & 8.28 & 1.34 & 0.10 & 0.09 & 5.29 & 3.30 & 0.11 & 0.07 & 6.71 & 2.15 \\
$w_1^1w_2^2$ & uniform & 0.25 & 0.19 & 0.11 & 15.28 & 7.73 & 0.10 & 0.10 & 7.63 & 5.63 & 0.14 & 0.12 & 11.04 & 4.38 \\
$w_1^2w_2^3$ & $w_1^0w_2^4$ & 0.25 & 0.17 & 0.13 & 8.14 & 2.37 & 0.30 & 0.20 & 5.74 & 2.01 & 0.27 & 0.07 & 6.87 & 1.56 \\
$w_1^3w_2^1$ & $w_1^1w_2^1$ & 0.33 & 0.34 & 0.04 & 14.34 & 1.90 & 0.29 & 0.16 & 10.30 & 7.57 & 0.28 & 0.07 & 13.71 & 4.19 \\
$w_1^0w_2^1$ & uniform & 0.50 & 0.41 & 0.12 & 24.03 & 1.90 & 0.42 & 0.13 & 24.51 & 1.53 & 0.45 & 0.11 & 25.71 & 1.83 \\
$w_1^1w_2^0$ & uniform & 0.50 & 0.43 & 0.12 & 23.43 & 1.67 & 0.45 & 0.14 & 23.86 & 2.30 & 0.47 & 0.13 & 25.16 & 2.17 \\
$w_1^1w_2^1$ & $w_1^0w_2^0$ & 0.50 & 0.33 & 0.15 & 21.03 & 1.88 & 0.29 & 0.18 & 19.08 & 5.50 & 0.32 & 0.14 & 20.24 & 2.99 \\
$w_1^3w_2^1$ & $w_1^3w_2^2$ & 0.67 & 0.58 & 0.29 & 21.59 & 13.13 & 0.67 & 0.22 & 8.95 & 3.97 & 0.63 & 0.23 & 13.96 & 6.65 \\
$w_1^2w_2^1$ & $w_1^2w_2^2$ & 0.75 & 0.79 & 0.16 & 12.37 & 8.59 & 0.71 & 0.23 & 12.04 & 5.99 & 0.66 & 0.17 & 12.92 & 5.37 \\
$w_1^4w_2^1$ & $w_1^6w_2^3$ & 0.88 & 0.76 & 0.46 & 21.04 & 14.34 & 0.77 & 0.33 & 10.58 & 3.04 & 0.81 & 0.30 & 10.78 & 2.65 \\
$w_1^1w_2^1$ & $w_1^1w_2^1$ & 1.00 & 0.80 & 0.15 & 39.48 & 7.04 & 0.75 & 0.25 & 35.65 & 12.11 & 0.92 & 0.22 & 51.91 & 15.17 \\
\bottomrule
\end{tabular}


==> images/toypotential_table_of_results_large.tex <==
\begin{tabular}{lll|rr|rr|rr|rr|rr|rr}
\toprule
monomial & prior & $\lambda$ & \multicolumn{4}{r}{MCMC} & \multicolumn{4}{r}{SGLD ($\epsilon=0.0001$)} & \multicolumn{4}{r}{SGLD ($\epsilon=0.0005$)} \\
 &  &  & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$\hat{\nu}^{\beta^*}$} & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$\hat{\nu}^{\beta^*}$} & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$\hat{\nu}^{\beta^*}$} \\
 &  &  & mean & std & mean & std & mean & std & mean & std & mean & std & mean & std \\
\midrule
$w_1^1w_2^3$ & $w_1^0w_2^0$ & 0.17 & 0.12 & 0.04 & 0.17 & 0.03 & 0.10 & 0.09 & 0.11 & 0.07 & 0.11 & 0.07 & 0.14 & 0.05 \\
$w_1^1w_2^3$ & $w_1^1w_2^0$ & 0.17 & 0.17 & 0.01 & 0.17 & 0.01 & 0.14 & 0.10 & 0.14 & 0.07 & 0.16 & 0.05 & 0.18 & 0.04 \\
$w_1^1w_2^2$ & $w_1^0w_2^0$ & 0.25 & 0.19 & 0.11 & 0.32 & 0.16 & 0.10 & 0.10 & 0.16 & 0.12 & 0.14 & 0.12 & 0.23 & 0.09 \\
$w_1^2w_2^3$ & $w_1^0w_2^4$ & 0.25 & 0.17 & 0.13 & 0.17 & 0.05 & 0.30 & 0.20 & 0.12 & 0.04 & 0.27 & 0.07 & 0.14 & 0.03 \\
$w_1^3w_2^1$ & $w_1^1w_2^1$ & 0.33 & 0.34 & 0.04 & 0.30 & 0.04 & 0.29 & 0.16 & 0.22 & 0.16 & 0.28 & 0.07 & 0.29 & 0.09 \\
$w_1^0w_2^1$ & $w_1^0w_2^0$ & 0.50 & 0.41 & 0.12 & 0.50 & 0.04 & 0.42 & 0.13 & 0.51 & 0.03 & 0.45 & 0.11 & 0.54 & 0.04 \\
$w_1^1w_2^0$ & $w_1^0w_2^0$ & 0.50 & 0.43 & 0.12 & 0.49 & 0.03 & 0.45 & 0.14 & 0.50 & 0.05 & 0.47 & 0.13 & 0.53 & 0.05 \\
$w_1^1w_2^1$ & $w_1^0w_2^0$ & 0.50 & 0.33 & 0.15 & 0.44 & 0.04 & 0.29 & 0.18 & 0.40 & 0.12 & 0.32 & 0.14 & 0.42 & 0.06 \\
$w_1^3w_2^1$ & $w_1^3w_2^2$ & 0.67 & 0.58 & 0.29 & 0.45 & 0.28 & 0.67 & 0.22 & 0.19 & 0.08 & 0.63 & 0.23 & 0.29 & 0.14 \\
$w_1^2w_2^1$ & $w_1^2w_2^2$ & 0.75 & 0.79 & 0.16 & 0.26 & 0.18 & 0.71 & 0.23 & 0.25 & 0.13 & 0.66 & 0.17 & 0.27 & 0.11 \\
$w_1^4w_2^1$ & $w_1^6w_2^3$ & 0.88 & 0.76 & 0.46 & 0.44 & 0.30 & 0.77 & 0.33 & 0.22 & 0.06 & 0.81 & 0.30 & 0.23 & 0.06 \\
$w_1^1w_2^1$ & $w_1^1w_2^1$ & 1.00 & 0.80 & 0.15 & 0.83 & 0.15 & 0.75 & 0.25 & 0.75 & 0.25 & 0.92 & 0.22 & 1.09 & 0.32 \\
\bottomrule
\end{tabular}


==> images/toypotential_table_of_results_small.tex <==
\begin{tabular}{lllrrrrrrrrrrrr}
\toprule
monomial & prior & $\lambda$ & \multicolumn{4}{r}{MCMC} & \multicolumn{4}{r}{SGLD ($\epsilon=0.0001$)} & \multicolumn{4}{r}{SGLD ($\epsilon=0.0005$)} \\
 &  &  & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$V_n^{\beta^*}/2$} & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$V_n^{\beta^*}/2$} & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$V_n^{\beta^*}/2$} \\
 &  &  & mean & std & mean & std & mean & std & mean & std & mean & std & mean & std \\
\midrule
$w_1^1w_2^3$ & uniform & 0.17 & 0.12 & 0.04 & 8.28 & 1.34 & 0.10 & 0.09 & 5.29 & 3.30 & 0.11 & 0.07 & 6.71 & 2.15 \\
$w_1^1w_2^2$ & uniform & 0.25 & 0.19 & 0.11 & 15.28 & 7.73 & 0.10 & 0.10 & 7.63 & 5.63 & 0.14 & 0.12 & 11.04 & 4.38 \\
$w_1^0w_2^1$ & uniform & 0.50 & 0.41 & 0.12 & 24.03 & 1.90 & 0.42 & 0.13 & 24.51 & 1.53 & 0.45 & 0.11 & 25.71 & 1.83 \\
$w_1^1w_2^0$ & uniform & 0.50 & 0.43 & 0.12 & 23.43 & 1.67 & 0.45 & 0.14 & 23.86 & 2.30 & 0.47 & 0.13 & 25.16 & 2.17 \\
\bottomrule
\end{tabular}


==> images/toypotential_table_of_results_small_backup.tex <==
\begin{tabular}{|lll|rr|rr|rr|rr|rr|rr|}
\toprule
 &  & & \multicolumn{4}{r}{MCMC} & \multicolumn{4}{r}{SGLD ($\epsilon=0.0001$)} & \multicolumn{4}{r|}{SGLD ($\epsilon=0.0005$)} \\
 &  &  & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$V_n^{\beta^*}/2$} & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$V_n^{\beta^*}/2$} & \multicolumn{2}{r}{$\hat{\lambda}$} & \multicolumn{2}{r}{$V_n^{\beta^*}/2$} \\
 monomial&  prior&  $\lambda$ & mean & std & mean & std & mean & std & mean & std & mean & std & mean & std \\
\midrule
$w_1^1w_2^1$ & $w_1^0w_2^0$ & 0.50 & 0.33 & 0.15 & 21.03 & 1.88 & 0.31 & 0.19 & 20.11 & 5.62 & 0.43 & 0.28 & 26.34 & 13.27 \\
 & $w_1^1w_2^1$ & 1.00 & 0.80 & 0.15 & 39.48 & 7.04 & 0.75 & 0.20 & 34.61 & 6.70 & 1.05 & 0.23 & 59.55 & 20.28 \\
$w_1^1w_2^3$ & $w_1^1w_2^0$ & 0.17 & 0.17 & 0.01 & 8.03 & 0.36 & 0.18 & 0.14 & 8.79 & 6.00 & 0.17 & 0.05 & 9.07 & 1.78 \\
$w_1^2w_2^1$ & $w_1^2w_2^2$ & 0.75 & 0.79 & 0.16 & 12.37 & 8.59 & 0.77 & 0.27 & 16.88 & 16.02 & 0.69 & 0.19 & 14.72 & 6.64 \\
$w_1^2w_2^3$ & $w_1^0w_2^4$ & 0.25 & 0.17 & 0.13 & 8.14 & 2.37 & 0.31 & 0.20 & 6.08 & 1.97 & 0.25 & 0.06 & 7.22 & 1.59 \\
$w_1^3w_2^1$ & $w_1^1w_2^1$ & 0.33 & 0.34 & 0.04 & 14.34 & 1.90 & 0.31 & 0.13 & 9.08 & 3.48 & 0.31 & 0.04 & 16.73 & 5.98 \\
 & $w_1^3w_2^2$ & 0.67 & 0.58 & 0.29 & 21.59 & 13.13 & 0.69 & 0.22 & 10.68 & 5.86 & 0.73 & 0.15 & 14.56 & 8.90 \\
$w_1^4w_2^1$ & $w_1^6w_2^3$ & 0.88 & 0.76 & 0.46 & 21.04 & 14.34 & 0.81 & 0.33 & 10.79 & 3.04 & 0.84 & 0.29 & 11.05 & 2.61 \\
\bottomrule
\end{tabular}

